Correspondence-Free SE(3) Point Cloud Registration in RKHS via Unsupervised Equivariant Learning

This paper introduces a robust unsupervised SE(3) point cloud registration method that operates without requiring point correspondences. The method frames point clouds as functions in a reproducing kernel Hilbert space (RKHS), leveraging SE(3)-equivariant features for direct feature space registration. A novel RKHS distance metric is proposed, offering reliable performance amidst noise, outliers, and asymmetrical data. An unsupervised training approach is introduced to effectively handle limited ground truth data, facilitating adaptation to real datasets. The proposed method outperforms classical and supervised methods in terms of registration accuracy on both synthetic (ModelNet40) and real-world (ETH3D) noisy, outlier-rich datasets. To our best knowledge, this marks the first instance of successful real RGB-D odometry data registration using an equivariant method. The code is available at {https://sites.google.com/view/eccv24-equivalign}

==> 06_limitation.tex <==

\section{Limitations}
% Limitations involve a long training time (a week for the full ModelNet) and suboptimal performances under large initial angles with low overlap. First, with the unsupervised training scheme, the curriculum learning strategy is required to bootstrap the training process at the cost of longer training time from smaller to larger rotations. In practice, the training on the ModelNet full dataset  and ETH3D takes a week and a day, respectively. Second, without supervision on the overlap, there is a performance decrease on the low-overlapped registration. As in Table~\ref{exp_modelnet_benchmark}, when the overlapped region is as low as 60\%, the proposed method has a decrease in the registration accuracy. 



==> tabs/01_modelnet_tables.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\small
\begin{tabular}{l|c|c|c|c|c|c|c}
\toprule 

%top level
% \multicolumn{8}{c}{
% \zm{Results 1}
% } \\
% \midrule


\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Type 
}   & \multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Method 
}  &  \multicolumn{3}{c}{Test Init Angle $<45^{\circ} $} & \multicolumn{3}{c}{Test Init Angle $<90^{\circ} $} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
&& $\sigma = 0, \gamma = 0$ & $\sigma = 0.01, \gamma = 0$ & $\sigma = 0.01, \gamma = 20\%$   & $\sigma = 0, \gamma = 0$ & $\sigma = 0.01, \gamma = 0$ & $\sigma = 0.01, \gamma = 20\%$ \\
\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Non-Learning \bf
%}
} 
& ICP & 0.25  & 0.37 & 0.62 &34.52 &
35.72 &  39.69\\
&GICP & 0.49 &0.45 &0.74&42.33& 43.64 &37.82 \\
& Geometric-CVO & 6.48 & 6.37 &  5.20 &  30.15 & 25.98 & 27.34\\
\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Invariant Features%}
} & FPFH + RANSAC &0.00&42.20&42.45&0.00
&85.40&85.34\\
& FPFH + FGR &0.04&1.22&18.72&0.14&4.83&41.45 \\
\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Equivariant Features
%}
}  & E2PN &1.46&3.70&6.75&1.42&3.17& 7.59 \\
&\equivcvo &0.29&
1.12 &
4.02&
1.07 &
2.70&
4.77  \\


%%% Begin of the second table
\midrule
% \multicolumn{8}{c}{
% \zm{Results 2}
% } \\
\midrule

\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Type 
}   & \multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Method 
}  &  \multicolumn{3}{c}{Test Init Angle $<45^{\circ} $} & \multicolumn{3}{c}{Test Init Angle $<90^{\circ} $} \\ 
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
&  & crop $5\%$ & crop $10\%$ & crop $20\%$   & crop $5\%$ & crop $10\%$ & crop $20\%$ \\
\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Non-Learning \bf
%}
} 
& ICP & 1.21 & 1.84 & 4.61 &38.04 &
41.25 &  42.00\\
&GICP & 1.17&2.51&1.26&32.96
&37.14&41.27 \\
& Geometric-CVO & 9.40 & 11.16 & 16.08 & 31.83 & 40.46 & 47.04 \\
\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Invariant Features%}
} & FPFH + RANSAC &42.83&42.75&43.10&85.89
&86.17&85.74\\
& FPFH + FGR &53.88&57.69&77.31&67.42&80.10&90.87 \\
\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Equivariant Features
%}
}  & E2PN &14.80&22.31
&18.76&24.19&18.05&21.80 \\
&\equivcvo &2.69&
7.07 &
14.48&
8.76 &
14.80&
30.10  \\
\bottomrule
\end{tabular}
}
\caption{
\zm{
\textbf{Rotation Error Analysis on the ModelNet Dataset:} (Top) Comparative performance of baselines under varying noise and outlier conditions. $\sigma$ is the variance of the Gaussian noise applied on the surface normal direction of each point. $\gamma$ is the ratio of points perturbed by uniformly distributed outliers. (Bottom) Baseline comparison across different crop ratios. }
}
\label{exp_modelnet_benchmark}
\FloatBarrier
\vspace{-20pt}
\end{table*}

==> tabs/03_eth3d_traj_table.tex <==
\begin{table}[!htbp]
\centering
\resizebox{\textwidth}{!}{
\footnotesize
\begin{tabular}{l|c|cc|cc|cc|cc}
\toprule 
\multirow{2}{*}{
Type 
}   & \multirow{ 2}{*}{Method}  &  \multicolumn{2}{c}{\texttt{sfm\_lab\_room\_1}, 262 frames} & \multicolumn{2}{c}{\texttt{plant\_1}, 69 frames} & \multicolumn{2}{c}{\texttt{table\_3}, 1046 frames} & \multicolumn{2}{c}{\texttt{sfm\_bench}, 659 frames} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}\\
&& {Rot. Error $(^{\circ})$} & {Trans. Error $(m)$} & {Rot. Error $(^{\circ})$} &  {Trans. Error $(m)$}  & {Rot. Error $(^{\circ})$} &  {Trans. Error $(m)$}  & {Rot. Error $(^{\circ})$} &  {Trans. Error $(m)$} \\ 

\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Non-Learning \bf
%}
} 
& ICP & 0.519	&0.031	&0.519	&0.011	&0.451	&0.011	&1.851	&0.031
\\
& GICP &\textbf{0.222}	&0.031	&0.471	&0.010	&0.394	&0.010	&\textbf{0.300}	&\textbf{0.007}
\\
& Geometric-CVO &0.243	&\textbf{0.006}	&\textbf{0.372}	&\textbf{0.007}	&0.325	&0.008	&0.643	&0.010

\\
\midrule
\multirow{ 2}{*}{
%\rotatebox[origin=l]{90}{
Invariant \\Features%}
} & FPFH + RANSAC &2.026	&0.099	&0.752	&0.088	&0.482	&0.074	&1.851	&0.076

\\
& FPFH + FGR &1.693	&0.037	&1.989	&0.034	&1.010	&0.024	&1.610	&0.036
\\
\midrule
%\multirow{ 2}{*}{
Equivariant Features
%}
%} 
%& E2PN &5.20& \textbf{0.00} 
%& NA & NA 
%\\
&\equivcvo & 0.247	&\textbf{0.006}	&\textbf{0.372}	&\textbf{0.007}	&\textbf{0.319}	&\textbf{0.007}	&0.581	&0.011
\\
\bottomrule
\end{tabular}
}
\caption{
\textbf{ETH3D  SE(3) Odometry Test Results per Sequence:} This table shows the pairwise registration errors per ETH3D sequence. 
One of the baselines, E2PN, is SE(3) equivariant, but the official implementation does not include translation predictions for this odometry experiment and thus is not included in this table. Among competing baselines, \equivcvo achieves lower rotation and translation errors in   two of the four test sequences. 
}
\label{appendix_eth3d_benchmark}
% \FloatBarrier
%\vspace{-25pt}
\end{table}
